Membership-based Manoeuvre Negotiation in Autonomous and Safety-critical Vehicular Systems

A fault-tolerant negotiation-based intersection crossing protocol is presented. Rigorous analytic proofs are used for demonstrating the correctness and fault-tolerance properties. Experimental results validate the correctness proof via detailed computer simulations and provide a preliminary evaluation of the system performances. The results are compared to the ones that can be achieved via a risk estimator with and without combining the proposed protocol. Our fault model considers packet-loss, noisy sensory information and malicious driving. Our preliminary results show a reduction in the number of dangerous situations and vehicle collisions.

==> include/Obsolete.tex <==
\Subsection{Uncertainty in Response Delays}
%May be used to explain the constants
 A constant $T_D$ is introduced to put a bound on the acceptable transmission delay. A bound is needed to ensure liveliness in the presence of communication failures like packet loss. For instance, if the request packet is lost then the requesting agent would have to wait forever to receive replies, because it is impossible for a requesting agent to determine if messages have been lost or otherwise delayed.
 
 An agent wishing to change the traffic priorities will have to wait at most $2T_D$ time units after sending a request for the final reply. Any answer arriving later than that will be ignored by the requesting vehicle. A new request will be initiated if all expected answers were not received. Unpredictable transmission delays, processing times and other factors that contribute to latency add additional uncertainty to the point in time when the final message will arrive. This also leads to an uncertainty to when the requested vehicle will reach and exit the critical section, see Figure \ref{fig:timeline}.
 A vehicle that gets granted immediately will in our model reach the intersection faster than if it had to wait for a while for all replies. This is because a vehicle will not change its intention to go until it is granted, and the speed model for having the intention to stop drops quicker to a slower speed than the corresponding speed model for the intention to go. The speed models use constant acceleration which means that time to the intersection (TTI) can be computed as
 \begin{equation}
     TTI = \int^{0}_{d}\frac{ds}{v} = constv+constacc
 \end{equation}
 \todo{Finish this equation}
 
 \begin{figure}
    \centering
    \includegraphics[scale=0.7]{figure/Time_line_request.png}
    \caption{A time line representation of when a requesting vehicle can be granted after having sent a request at $t=T_{Early}$ and the time it correspondingly enters and exits the critical section. A granted vehicle will change its intention from stop to go which means that it will reach the intersection and leave it faster than if it has to wait longer for replies. We consider the vehicle to be inside the critical section during the whole red interval, from the earliest predicted entry to the latest predicted exit, since the exact time of receiving permission within the green interval is unknown.}
    \label{fig:timeline}
\end{figure}
 
 \Subsection{Deviations from the speed model}
 
 A vehicle may deviate from the speed model which can be accounted for by applying a gap policy to the gaps between the occupation intervals. This gap policy may be deterministic or non-deterministic function that given a gap as input returns ''safe'' or ''dangerous'' corresponding to a safe respectively dangerous gap. Choosing a deterministic policy means that the acceptable time gap between two intervals will have to be either fixed or depend on the situation. This may potentially lead to a deadlock since two identical situations will give rise to the same acceptable gap and if the first situation doesn't change than neither will the second following and so on.
 
 A non-deterministic policy must define the acceptable gap as a random variable. For the task described in this report it would be suitable to choose the gap acceptance function to be a logistic function like in~\cite{GapModel},
 \begin{equation}\label{eq:speed_model}
     Y=\frac{1}{1+e^{b(a-x)}}.
 \end{equation}
 Large time gaps will then have a large likelihood of being considered acceptable and the opposite for small gaps.
 
 
 \Subsection{Intervals}
 
 . have to determine whether to grant or deny the requesting vehicle. This decision depends on the predicted occupation intervals, where an overlap of the intervals signifies an overlap in time of using the critical section. These intervals are evaluated and compared in the function $\noPriorityViolation$ which is called by an agent receiving a request to decide whether to GRANT or DENY.
 
 Two approaches to implementing $\noPriorityViolation$ have been developed in this project, one that assumes fixed priorities and one that assumes a dynamic priority order. These approaches are presented in \ref{sec:nPV_static} and \ref{sec:npv_dynamic}.


\Subsection{$\noPriorityViolation$ with Static priorities}
\label{sec:nPV_static}
\todo[inline]{Edit}
A deterministic implementation of $\noPriorityViolation$ could be based on occupancy prediction. This approach would involve making an over-estimation of a vehicle's position for consecutive time frames. The result is one area per time interval so that the vehicle cannot be outside the predicted area during the given time interval. One such approach is presented by~\cite{Occupancy} where both physical and legal constraints are applied to predict vehicle motion.
Further constraints can be applied if multiple vehicles are present in a traffic scene~\cite{IntentionAwareOccupancy}. Some vehicles may then slow down others if the road is narrow, making it impossible to overtake the slow vehicle and thereby adding further limitations to the speed of the following vehicles.
An overlap in any of the areas for the consecutive time frames signifies a possible priority violation. $\noPriorityViolation$ would therefore have to be implemented to return true only if no overlaps exist in the predicted areas for time intervals from the current time until the vehicle asking for permission has left the intersection (the rear part of the area does not overlap with the intersection).

\Subsection{$\noPriorityViolation$ with Dynamic priorities}
\label{sec:npv_dynamic}
\todo[inline]{Edit}
The presented approach in Section \ref{sec:nPV_static} should be able to predict all priority violations since it is relying on what is physically possible. However, the approach is not efficient regarding throughput in normal traffic situations where most vehicles follow normal trajectory and speed patterns. We therefore decided to employ a non-deterministic solution based on behaviour models and intersection occupation intervals. This approach requires predefined trajectories and speed models corresponding to going straight, turning left or right and stopping.  Following these patterns in position and speed enables making a prediction of when each vehicle will enter and exit the intersection. The smallest time gap with the ego vehicle's time interval and any others' can then be used as input to a gap-acceptance function. Using a \todo{or constant threshold}logistic function as a cumulative distribution function for the gaps that should be accepted was shown to perform well for cases of left turn across path~\cite{GapModel}. Parameters in the logistic function can be adjusted to fit the conditions in any particular intersection and it is the gap-model we intend to use.

This non-deterministic approach cannot guarantee that no priority violation will occur if vehicles show a deviating behaviour from the normal patterns and if the priorities are kept static. To ensure that priorities are not violated we could make them dynamic instead so that giving another vehicle a grant entails giving that vehicle a higher priority.



\Subsection{Grants based on negative time gaps}

 If a vehicle $a_i$ grants another vehicle $a_j$ based on a negative time gap, then there is no guarantee that $a_j$ will not be in the intersection when $a_i$ enters it. Crossing pedestrians or engine failure may for example cause $a_j$ to slow down and stop. The question is if rare deviation from normal driving should be accounted for by the manoeuvre negotiation protocol or if it should be detected by the risk estimator as unexpected behaviour.
 \todo[inline]{Needs to be revised}
 Adding the rule that a negative time gap leads to a DENY and that granting vehicles are not allowed to enter the critical section until the grant expires ensures that the granting vehicle will not be in the intersection when the granted vehicle enters it. However, this solution does not directly provide safety in the case where a granting vehicle arrives earlier at the intersection than predicted. Poor road conditions or faulty brakes can cause a vehicle that intended to slow down (to do a turn) to instead reach the intersection early. This is a problem in cold climates where unexpected ice patches cause a driver to lose control over the vehicle. One can argue that a safety margin can be added to the positive time gap which could solve the problem, but how would such a safety margin be determined to guarantee safety? Instead I propose that both these deviations from "normal" behaviour should be classified as environmentally caused deviations that should be detected by the risk estimator and not be considered by the manoeuvre negotiator (a safety margin would of course be added to the predicted occupancy intervals to increase the safety probability, but it cannot by itself guarantee that the vehicles will follow their intentions perfectly).
 
 
  \Subsection{Grant with restrictions}
 %One problem with having only one type of grant message is that if you want to guarantee safety then vehicles that are asked to change the priorities will have to reply with a DENY if the calculated time gap is negative.
 \todo[inline]{revise, this may not be necessary. Denying until leaving the intersection would have the same effect}
 One possible solution to making it safer to grant when there is a negative time gap is to add a third possible reply to a request: GRANT with restriction. To grant with restriction means to give the requesting vehicle a permission to perform the manoeuvre but only after the requested vehicle has left the critical section, that is, giving it a lower priority. This implies that if the requested vehicle has to stop in the critical section, then the granted vehicle will wait for it to leave before entering. The proposed solution does not depend on the risk estimator to detect the unexpected behaviour but instead on the established priority order.
 
 A normal GRANT indicates that the requested vehicle gives higher priority to the requesting vehicle, and a DENY that no change in priority will take place.
 
 \Subsection{Static vs Dynamic priorities}
 
 \Section{$\noPriorityViolation$ with Static priorities}
\label{sec:nPV_static}
\todo[inline]{Edit and rename}
A deterministic implementation of $\noPriorityViolation$ could be based on occupancy prediction. This approach would involve making an over-estimation of a vehicle's position for consecutive time frames. The result is one area per time interval so that the vehicle cannot be outside the predicted area during the given time interval. One such approach is presented by~\cite{Occupancy} where both physical and legal constraints are applied to predict vehicle motion.
Further constraints can be applied if multiple vehicles are present in a traffic scene~\cite{IntentionAwareOccupancy}. Some vehicles may then slow down others if the road is narrow, making it impossible to overtake the slow vehicle and thereby adding further limitations to the speed of the following vehicles.
An overlap in any of the areas for the consecutive time frames signifies a possible priority violation. $\noPriorityViolation$ would therefore have to be implemented to return true only if no overlaps exist in the predicted areas for time intervals from the current time until the vehicle asking for permission has left the intersection (the rear part of the area does not overlap with the intersection).



\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}[]
% 1st column
\node               at (0,6) {$t=1$};
\node[state] (s1_1) at (0,5) {$s_1$};
\node[mainstate] (s2_1) at (0,4) {$s_2$};
\node[state] (s3_1) at (0,3) {$s_3$};
\node[state] (s4_1) at (0,2) {$s_4$};
\node at (0,1) {$y_1$};
% 2nd column
\node               at (2,6) {$t=2$};
\node[mainstate] (s1_2) at (2,5) {$s_1$}
    edge[lightedge] (s1_1)
    edge[mainedge] (s2_1)
    edge[lightedge] (s3_1)
    edge[lightedge] (s4_1);
\node[state] (s2_2) at (2,4) {$s_2$}
    edge[lightedge] (s1_1)
    edge[lightedge] (s2_1)
    edge[lightedge] (s3_1)
    edge[lightedge] (s4_1);
\node[state] (s3_2) at (2,3) {$s_3$}
    edge[lightedge] (s1_1)
    edge[lightedge] (s2_1)
    edge[lightedge] (s3_1)
    edge[lightedge] (s4_1);
\node[state] (s4_2) at (2,2) {$s_4$}
    edge[lightedge] (s1_1)
    edge[lightedge] (s2_1)
    edge[lightedge] (s3_1)
    edge[lightedge] (s4_1);
\node at (2,1) {$y_2$};
% 3rd column
\node               at (4,6) {$t=3$};
\node[mainstate] (s1_3) at (4,5) {$s_1$}
    edge[mainedge]  (s1_2)
    edge[lightedge] (s2_2)
    edge[lightedge] (s3_2)
    edge[lightedge] (s4_2);
\node[state] (s2_3) at (4,4) {$s_2$}
    edge[lightedge] (s1_2)
    edge[lightedge] (s2_2)
    edge[lightedge] (s3_2)
    edge[lightedge] (s4_2);
\node[state] (s3_3) at (4,3) {$s_3$}
    edge[lightedge] (s1_2)
    edge[lightedge] (s2_2)
    edge[lightedge] (s3_2)
    edge[lightedge] (s4_2);
\node[state] (s4_3) at (4,2) {$s_4$}
    edge[lightedge] (s1_2)
    edge[lightedge] (s2_2)
    edge[lightedge] (s3_2)
    edge[lightedge] (s4_2);
\node at (4,1) {$y_2$};
\end{tikzpicture}
\end{center}
\caption{Trellis of the observation sequence $y_1$,$y_2$,$y_2$ for the above HMM. The thick arrows
indicate the most probable transitions. As an example, the transition
between state $s_1$ at time t=2 and state $s_4$ at time t=3 has probability
$\alpha_2(1)a_{14}b_4(y_2)$, where $\alpha_t(i)$ is the probability to be in
state $s_i$ at time t. }
\label{fig:HMM}
\end{figure}


\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}[]
% states
\node[state] (s1) at (0,2) {$s_1$}
    edge [loop above]  ();
\node[state] (s2) at (2,2) {$s_2$}
    edge [<-,bend right=45] node[auto,swap] {$a_{12}$} (s1)
    edge [->,bend left=45] (s1)
    edge [loop above] ();
\node[state] (s3) at (4,2) {$s_3$}
    edge [<-,bend right=45] (s2)
    edge [->,bend left=45] (s2)
    edge [loop above] ();
\node[state] (s4) at (6,2) {$s_4$}
    edge [<-,bend right=45] (s3)
    edge [->,bend left=45] (s3)
    edge [loop above] ();
% observations
\node[observation] (y1) at (2,0) {$y_1$}
    edge [lightedge] (s1)
    edge [lightedge] (s2)
    edge [lightedge] (s3)
    edge [lightedge] (s4);
\node[observation] (y2) at (4,0) {$y_2$}
    edge [lightedge] (s1)
    edge [lightedge] (s2)
    edge [lightedge] (s3)
    edge [lightedge] node[auto,swap] {$b_4(y_2)$} (s4);
\end{tikzpicture}
\end{center}
\caption{An HMM with 4 states which can emit 2 discrete symbols $y_1$ or $y_2$.
$a_{ij}$ is the probability to transition from state $s_i$ to state $s_j$.
$b_j(y_k)$ is the probability to emit symbol $y_k$ in state $s_j$.
In this particular HMM, states can only reach themselves or the adjacent state.}
\end{figure}

==> include/backmatter/PseudoCode2.tex <==
% CREATED BY DAVID FRISK, 2016
\newgeometry{left=.9in, right=.9in, top=.8in, bottom=.8in}

\chapter{Pseudo code for the Manoeuvre Negotiation protocol}

%\section{Full pseudo code for the explicit release extension}
\label{sec:Pseudo}



\begin{algorithm}[ht!]
	\begin{small}
		\textbf{Structures:}\\
		$Segment = (xs, xsh, xeh, xe)$\tcp*[r]{positions: start, start handoff, end handoff, end}
		$AgentState = (ta,x,v,a)$\tcp*[r]{timestamp, position, velocity, acceleration}
		$Agent = (aID,AS)$\tcp*[r]{agent ID, AgentState structure}
		$Membership = (tm,MO,\mathcal{SM})$\tcp*[r]{timestamp, MO flag, $\mathcal{SM}$ IDs of agents in the membership}
		\ \\
		\textbf{Variables:}\\
		$S \gets getSegmentData(sID())$\tcp*[r]{Segment registry}
		%$MO$\tcp*[r]{Maneuver Opportunity}
		%$\mathcal{SM}$\tcp*[r]{Set of agent IDs (Safety Membership set)}
		$\mathcal{MR} \gets \bot$\tcp*[r]{Membership registry}
		$T\_UPDATE$\tcp*[r]{Timer for periodic update of MR registries on the storage service}
		\ \\
		\textbf{Interfaces:}\\
		$sID()$: get segment ID\;
		$clock()$: read current time\;
		%$createTimer()$: create a new timer\;
		$startTimer(timer,delay)$: start named $timer$ for $delay$ time units\;
		$getSegmentData(sID)$: read Segment registry for segment $sID$ from storage servive\;
		$getARSet(sID)$: read all Agent registries for segment $sID$ from the storage service\;
		$storeMR(aID,MR)$: write $MR$ (Membership registry) for agent $aID$ on the storage service\;
		%$getUnsafeAgents(AR,t)$: obtain the set of agent IDs that are within distance $Z_2$ of the agent identified by $AR$, whose safety bubble might touch the joint safety bubble of that agent until $t$\;
		$getUnsafeAgents(AR,t)$: obtain a list of sets of agent IDs that have right-of-way and are within the distance $Z_2$ in respect to the agent identified by $AR$ for the different possible turns (defined by $getPossibleTurns(AR)$) for this agent\;
		$getReachableAgents(AR,t)$: obtain the set of agents IDs that will be within communication range of the agent identified by $AR$ until $t$ \;
		$getPossibleTurns(AR)$: obtain a list of possible turns for an agent\;
		\ \\
		\textbf{Initialization:}\\
		%$S \gets getSegmentData(sID())$\;
		%$\mathcal{MR} \gets \bot$\;
		%$T\_UPDATE \gets createTimer()$\;
		$startTimer(T\_UPDATE,T_M)$\;
		\ \\
		\textbf{upon} timer $T\_UPDATE$ expires, do
		\Begin{
			\textbf{let} $\mathcal{A} = getARSet(sID())$\;
			\ForEach{$AR$ in $\mathcal{A}$}{
				\If{$AR.AS.x > S.xsh \land AR.AS.x < S.xeh$}{
					\textbf{let} $t = clock()$\;
					\textbf{let} $\mathcal{U}=getUnsafeAgents(AR,t+T_M+2T_D+T_{MAN})$\;
					\textbf{let} $\mathcal{R}=getReachableAgents(AR,t+T_M+2T_D+T_{MAN})$\;
					\ForEach{turn \textnormal{in} getPossibleTurns(AR)}{
					\textbf{let} $t_{min} = min(\alpha.AS.ta : ( \alpha \in \mathcal{A}) \land (\alpha.aID \in \mathcal{U}[turn]))$\;
					\leIf{$\mathcal{U}[turn] \subset \mathcal{R}$}{$MR[turn] \gets (t_{min},\text{TRUE}, \mathcal{U})$}{$MR[turn] \gets (t_{min},\text{FALSE},\bot)$}
				    }	
					$storeMR(AR.aID,
				    MR)$\; %TODO check freshness of AR, something like min(AR.AS.ta: A.aID \in \mathcal{U}[turn]
					
				}
			}
			$startTimer(T\_UPDATE,T_M)$\;
		}
		
	\end{small}
	\caption{The membership algorithm.}
	\label{alg:membership}
\end{algorithm}
	
\begin{figure}[t!]
    \LinesNotNumbered
    %\DontPrintSemicolon
    \begin{framed}
    
    
	\begin{small}
		\textbf{Structures:}\\
		$AgentState = (ta,x,v,a)$\tcp*[r]{timestamp, position, velocity, acceleration}
		$Agent = (aID,AS)$\tcp*[r]{agent ID, AgentState structure}
		$AgentTag = (ts,aID,turn)$\tcp*[r]{timestamp, agent ID, intended turn}
		$Membership = (tm,MO,\mathcal{SM})$\tcp*[r]{timestamp, MO flag, $\mathcal{SM}$ set of agent IDs}
		$AgentTag = (aID, tt, turn)$\tcp*[r]{...}
		$Message = (t,type,(Agent,AgentTag))$\tcp*[r]{timestamp,message type, message data: Agent and AgentTag structures}
		
		\ \\
		\textbf{Variables:} \\
		$AR$\tcp*[r]{Agent registry} 
		$MR$\tcp*[r]{Membership registry}
		%$ts$\tcp*[r]{Starting time of a maneuver tentative} %Doesn't need to be a state variable
		$status \gets NORMAL$\tcp*[r]{NORMAL, GET, GRANT, TRYGET, GRANTGET, EXECUTE}
		$tag \gets \bot$\tcp*[r]{Unique tag for each maneuver}
		$grantID \gets \bot$\tcp*[r]{ID of the agent with an active GRANT}
		$\mathcal{M} \gets \bot$\tcp*[r]{Set of received messages}
		$\mathcal{D} \gets \bot$\tcp*[r]{Set of destination agent IDs}
		$\mathcal{R} \gets \bot$\tcp*[r]{Set of expected response agent IDs}
		$T\_UPDATE$\tcp*[r]{Timer for periodic AR update on storage service}
		$T\_RETRY$\tcp*[r]{Timer for retrying to get permission for maneuver}
		$T\_GRANT$\tcp*[r]{Timer for checking if a granted car has left the critical section}
		
		\ \\
		\textbf{Interfaces:}\\
		$aID()$: get agent ID\; \\
		$clock()$: read current time\; \\
		$position()$: read current agent position\; \\
		$velocity()$: read current agent velocity\; \\
		$acceleration()$: read current agent acceleration\; \\
		%$createTimer()$: create a new timer\;
		$startTimer(timer,delay)$: start named $timer$ for $delay$ time units\; \\
		$stopTimer(timer)$: stop named $timer$\; \\
		$storeAR(AR)$: write an $AR$ registry to the storage service \; \\
		$getMR(aID)$: read from the storage service the $MR$ for agent $aID$\; \\
		%\textbf{multicast} $\langle message \rangle$ \textbf{to} $\{D\}$: multicast $message$ to all nodes in $\{D\}$\; \\
		%\textbf{send} $\langle message \rangle$  \textbf{to} $destination$: \textcolor{red}{send $m$ to one-hop distance node $d$}\; \\
		$doManeuver(t)$: execute the maneuver until time instant $t$\; \\
		$noConflict(AR,t)$: check if conflicts with agent specified in $AR$ can be avoided until $t$\; \\
		$last()$: returns TRUE if $\mathcal{R} \cap D \cap MR.SM = \emptyset$, FALSE otherwise\; \\
		%$granted(aID)$: returns TRUE if $aID$ is the same as $grantID$, or FALSE otherwise\EMS{Why there is a need for this macro?} \EE{Replace with 'aID $\in$ grantID'}\;
		$precedes(rectag)$: returns TRUE if $rectag$ precedes current maneuver $tag$, or FALSE otherwise\; \\
		$hasLeftCriticalSection(aID)$: Check if the stored AR of agent aID reveals that the agent has left the critical section\; 
		
		%\ \\
		%\textbf{Initialization:}\\
		%$(status, grantID, tag) \gets \bot, \bot)$\;
		%$(\mathcal{M}, \mathcal{D}, \mathcal{R}) \gets (\bot, \bot, \bot)$
		
	\end{small}
	
	\caption{Structures, variables and interfaces for the manoeuvre negotiation protocol}
	\label{alg:defs}
	\end{framed}
\end{figure}

\newgeometry{left=.9in, right=.9in, top=.1in, bottom=.8in}
\begin{algorithm}[ht!]
	\begin{footnotesize}
		
		\textbf{do forever} 
	    \Begin{
		    %\textbf{write}$(AR, (aID(),(clock(), position(), velocity(), acceleration()))$\;
		    $AR \gets (aID(),(clock(), position(), velocity(), acceleration()))$\;
			$storeAR(AR)$\;
			$MR \gets getMR(aID())$\;
			%\lIf{$status \in \{GET, TRYGET\}$}{$MR \gets MR[tag.turn]$}
			\If(\tcp*[f]{All expected answers received}){$status=GET \land last()$}{
				$stopTimer(T\_RETRY)$\tcp*[r]{No need for a retry}
				\lIf{$\nexists {m \in \mathcal{M}}:m.type = DENY$}{
				    $status \gets EXECUTE$
				}\Else{
					$status \gets TRYGET$\;
					\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
					$startTimer(T\_RETRY,T_A)$\;
				}
			}
			\If{$status=EXECUTE \land hasLeftCriticalSection(aID())$}{
				\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\tcp*[r]{Explicit release}
				$status \gets NORMAL$\;
			}
		}
		
		\textbf{upon} $tryManeuver(turn)$ is invoked, do
		\Begin{				                              \lIf{$status \in \{NORMAL, GRANT\}$}{$tag \gets (clock(),aID(),turn)$}
			\uIf{$status \in \{NORMAL, TRYGET\}$}{
			    \textbf{let} $ts = clock()$\;
				$(status,AR,MR) \gets (TRYGET,(aID(), (ts,position(),velocity(),acceleration()),getMR(aID()))$\;
				\uIf{$(ts < MR[turn].tm + 2T_M \land MR[turn].MO)$}{
					$(\mathcal{M},\mathcal{D},\mathcal{R}, status) \gets (\bot,MR[turn].\mathcal{SM},MR[turn].\mathcal{SM}, GET)$\;
					\textbf{multicast} $\langle ts, GET, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
					$startTimer(T\_RETRY,2T_D)$\;
				}
				\lElse{$startTimer(T\_RETRY,T_A)$}
			}
			\lElseIf{$status=GRANT$}{$status \gets GRANTGET$}
		}
		\textbf{upon} timer $T\_RETRY$ expires
		\Begin{
			\If{$status=GET$}{
				$status \gets TRYGET$\;
				\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
				$startTimer(T\_RETRY,2T_D)$\;
			}
			$tryManeuver(tag.turn)$\;
		}
		
		\textbf{upon} timer $T\_GRANT$ expires
		\Begin{
		    \textbf{let} $prevStatus = status$\;
			\If{$status \in \{GRANT, GRANTGET\} \land hasLeftCriticalSection(grantID)$}{$(status,grantID) \gets (NORMAL,\bot)$\; 
			    \lIf{$prevStatus = GRANTGET$}{
				    $tryManeuver()$}
		    }
			\lIf{$status \in \{GRANT, GRANTGET\}$}{$startTimer(T\_{GRANT},T_{Recover}$)}
			
		}
		
		\textbf{upon} message $m$ received at time $tr$
		\Begin{
			\If(\tcp*[f]{Message is timely}){$tr-m.t \leq T_D$}{
				\lIf{$m.type \in \{GRANT,DENY\} \land status=GET$}{
					$(\mathcal{M},\mathcal{R}) \gets (\mathcal{M} \cup \{m\},\mathcal{R} \setminus \{m.AR.aID\} )$
				}
				\uElseIf{$m.type=GET$}{
					\uIf{$noConflict(m.AR,m.AR.AS.ta + 2T_D + T_{MAN}) \land \newline (status\in\{NORMAL,TRYGET\} \lor (status=GET \land precedes(m.tag)) \lor \newline (status\in\{GRANT,GRANTGET\} \land grantID = m.AR.aID) )$}{
						\lIf{$status=NORMAL$}{$(status,grantID) \gets (GRANT,m.AR.aID)$}
						\ElseIf{$status \in \{GET,TRYGET\}$}{
							$stopTimer(T\_RETRY)$\;
							\lIf{$status=GET$}{\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$}
							$(status,grantID) \gets (GRANTGET,m.AR.aID)$\;
						}
						\textbf{send} $\langle tr, GRANT, \bot \rangle$ \textbf{to} $m.AR.aID$\;
						$startTimer(T\_GRANT, m.AR.AS.t + 2T_D + T_{MAN} - clock())$\; 
					}
					\lElse{\textbf{send} $\langle tr, DENY, \bot \rangle$ \textbf{to} $m.AR.aID$}
				}
				\ElseIf{$m.type=RELEASE \land status \in \{GRANT,GRANTGET\} \land grantID = m.AR.aID $}{
					$stopTimer(T\_GRANT)$\tcp*[r]{No need checking if an agent has left}
					$grantID \gets \bot$\;
					\lIf{$status=GRANT$}{$status \gets NORMAL$}
					\If{$status=GRANTGET$}{
						$status \gets TRYGET$\;
						$tryManeuver(tag.turn)$\;
					}
				}
			}
		}
		
	\end{footnotesize}
	\caption{The Manoeuvre Negotiation protocol}
	\label{alg:agent-events}
\end{algorithm}



==> include/backmatter/PseudoCode_old.tex <==
\newgeometry{left=.9in, right=.9in, top=.8in, bottom=.8in}

\chapter{Pseudo code for the Manoeuvre Negotiation protocol}

%\section{Full pseudo code for the explicit release extension}
\label{sec:Pseudoold}


\begin{algorithm}[ht!]
	\begin{small}
		\textbf{Structures:}\\
		$Segment = (xs, xsh, xeh, xe)$\tcp*[r]{positions: start, start handoff, end handoff, end}
		$AgentState = (ta,x,v,a)$\tcp*[r]{timestamp, position, velocity, acceleration}
		$Agent = (aID,AS)$\tcp*[r]{agent ID, AgentState structure}
		$Membership = (tm,MO,\mathcal{SM})$\tcp*[r]{timestamp, MO flag, $\mathcal{SM}$ IDs of agents in the membership}
		\ \\
		\textbf{Variables:}\\
		$S \gets getSegmentData(sID())$\tcp*[r]{Segment registry}
		%$MO$\tcp*[r]{Maneuver Opportunity}
		%$\mathcal{SM}$\tcp*[r]{Set of agent IDs (Safety Membership set)}
		$\mathcal{MR} \gets \bot$\tcp*[r]{Membership registry}
		$T\_UPDATE$\tcp*[r]{Timer for periodic update of MR registries on the storage service}
		\ \\
		\textbf{Interfaces:}\\
		$sID()$: get segment ID\;
		$clock()$: read current time\;
		%$createTimer()$: create a new timer\;
		$startTimer(timer,delay)$: start named $timer$ for $delay$ time units\;
		$getSegmentData(sID)$: read Segment registry for segment $sID$ from storage servive\;
		$getARSet(sID)$: read all Agent registries for segment $sID$ from the storage service\;
		$storeMR(aID,MR)$: write $MR$ (Membership registry) for agent $aID$ on the storage service\;
		%$getUnsafeAgents(AR,t)$: obtain the set of agent IDs that are within distance $Z_2$ of the agent identified by $AR$, whose safety bubble might touch the joint safety bubble of that agent until $t$\;
		$getUnsafeAgents(AR,t)$: obtain a list of sets of agent IDs that have right-of-way and are within the distance $Z_2$ in respect to the agent identified by $AR$ for the different possible turns (defined by $getPossibleTurns(AR)$) for this agent\;
		$getReachableAgents(AR,t)$: obtain the set of agents IDs that will be within communication range of the agent identified by $AR$ until $t$ \;
		$getPossibleTurns(AR)$: obtain a list of possible turns for an agent\;
		\ \\
		\textbf{Initialization:}\\
		%$S \gets getSegmentData(sID())$\;
		%$\mathcal{MR} \gets \bot$\;
		%$T\_UPDATE \gets createTimer()$\;
		$startTimer(T\_UPDATE,T_M)$\;
		\ \\
		\textbf{upon} timer $T\_UPDATE$ expires, do
		\Begin{
			\textbf{let} $\mathcal{A} = getARSet(sID())$\;
			\ForEach{$AR$ in $\mathcal{A}$}{
				\If{$AR.AS.x > S.xsh \land AR.AS.x < S.xeh$}{
					\textbf{let} $t = clock()$\;
					\textbf{let} $\mathcal{U}=getUnsafeAgents(AR,t+T_M+2T_D+T_{MAN})$\;
					\textbf{let} $\mathcal{R}=getReachableAgents(AR,t+T_M+2T_D+T_{MAN})$\;
					\ForEach{turn \textnormal{in} getPossibleTurns(AR)}{
					\textbf{let} $t_{min} = min(\alpha.AS.ta : ( \alpha \in \mathcal{A}) \land (\alpha.aID \in \mathcal{U}[turn]))$\;
					\leIf{$\mathcal{U}[turn] \subset \mathcal{R}$}{$MR[turn] \gets (t_{min},\text{TRUE}, \mathcal{U})$}{$MR[turn] \gets (t_{min},\text{FALSE},\bot)$}
				    }	
					$storeMR(AR.aID,
				    MR)$\; %TODO check freshness of AR, something like min(AR.AS.ta: A.aID \in \mathcal{U}[turn]
					
				}
			}
			$startTimer(T\_UPDATE,T_M)$\;
		}
		
	\end{small}
	\caption{The membership algorithm.}
	\label{alg:membership}
\end{algorithm}
	
\begin{figure}[t!]
    \LinesNotNumbered
    %\DontPrintSemicolon
    \begin{framed}
    
    
	\begin{small}
		\textbf{Structures:}\\
		$AgentState = (ta,x,v,a)$\tcp*[r]{timestamp, position, velocity, acceleration}
		$Agent = (aID,AS)$\tcp*[r]{agent ID, AgentState structure}
		$AgentTag = (ts,aID,turn)$\tcp*[r]{timestamp, agent ID, intended turn}
		$Membership = (tm,MO,\mathcal{SM})$\tcp*[r]{timestamp, MO flag, $\mathcal{SM}$ set of agent IDs}
		$AgentTag = (aID, tt, turn)$\tcp*[r]{...}
		$Message = (t,type,(Agent,AgentTag))$\tcp*[r]{timestamp,message type, message data: Agent and AgentTag structures}
		
		\ \\
		\textbf{Variables:} \\
		$AR$\tcp*[r]{Agent registry} 
		$MR$\tcp*[r]{Membership registry}
		%$ts$\tcp*[r]{Starting time of a maneuver tentative} %Doesn't need to be a state variable
		$status \gets NORMAL$\tcp*[r]{NORMAL, GET, GRANT, TRYGET, GRANTGET, EXECUTE}
		$tag \gets \bot$\tcp*[r]{Unique tag for each maneuver}
		$grantID \gets \bot$\tcp*[r]{ID of the agent with an active GRANT}
		$\mathcal{M} \gets \bot$\tcp*[r]{Set of received messages}
		$\mathcal{D} \gets \bot$\tcp*[r]{Set of destination agent IDs}
		$\mathcal{R} \gets \bot$\tcp*[r]{Set of expected response agent IDs}
		$T\_UPDATE$\tcp*[r]{Timer for periodic AR update on storage service}
		$T\_RETRY$\tcp*[r]{Timer for retrying to get permission for maneuver}
		$T\_GRANT$\tcp*[r]{Timer for checking if a granted car has left the critical section}
		
		\ \\
		\textbf{Interfaces:}\\
		$aID()$: get agent ID\; \\
		$clock()$: read current time\; \\
		$position()$: read current agent position\; \\
		$velocity()$: read current agent velocity\; \\
		$acceleration()$: read current agent acceleration\; \\
		%$createTimer()$: create a new timer\;
		$startTimer(timer,delay)$: start named $timer$ for $delay$ time units\; \\
		$stopTimer(timer)$: stop named $timer$\; \\
		$storeAR(AR)$: write an $AR$ registry to the storage service \; \\
		$getMR(aID)$: read from the storage service the $MR$ for agent $aID$\; \\
		%\textbf{multicast} $\langle message \rangle$ \textbf{to} $\{D\}$: multicast $message$ to all nodes in $\{D\}$\; \\
		%\textbf{send} $\langle message \rangle$  \textbf{to} $destination$: \textcolor{red}{send $m$ to one-hop distance node $d$}\; \\
		$doManeuver(t)$: execute the maneuver until time instant $t$\; \\
		$noConflict(AR,t)$: check if conflicts with agent specified in $AR$ can be avoided until $t$\; \\
		$last()$: returns TRUE if $\mathcal{R} \cap D \cap MR.SM = \emptyset$, FALSE otherwise\; \\
		%$granted(aID)$: returns TRUE if $aID$ is the same as $grantID$, or FALSE otherwise\EMS{Why there is a need for this macro?} \EE{Replace with 'aID $\in$ grantID'}\;
		$precedes(rectag)$: returns TRUE if $rectag$ precedes current maneuver $tag$, or FALSE otherwise\; \\
		$hasLeftCriticalSection(aID)$: Check if the stored AR of agent aID reveals that the agent has left the critical section\; 
		
		%\ \\
		%\textbf{Initialization:}\\
		%$(status, grantID, tag) \gets \bot, \bot)$\;
		%$(\mathcal{M}, \mathcal{D}, \mathcal{R}) \gets (\bot, \bot, \bot)$
		
	\end{small}
	
	\caption{Structures, variables and interfaces for the manoeuvre negotiation protocol}
	\label{alg:defs}
	\end{framed}
\end{figure}

\newgeometry{left=.9in, right=.9in, top=.1in, bottom=.8in}
\begin{algorithm}[ht!]
	\begin{footnotesize}
		
		\textbf{do forever} 
	    \Begin{
		    %\textbf{write}$(AR, (aID(),(clock(), position(), velocity(), acceleration()))$\;
		    $AR \gets (aID(),(clock(), position(), velocity(), acceleration()))$\;
			$storeAR(AR)$\;
			$MR \gets getMR(aID())$\;
			%\lIf{$status \in \{GET, TRYGET\}$}{$MR \gets MR[tag.turn]$}
			\If(\tcp*[f]{All expected answers received}){$status=GET \land last()$}{
				$stopTimer(T\_RETRY)$\tcp*[r]{No need for a retry}
				\lIf{$\nexists {m \in \mathcal{M}}:m.type = DENY$}{
				    $status \gets EXECUTE$
				}\Else{
					$status \gets TRYGET$\;
					\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
					$startTimer(T\_RETRY,T_A)$\;
				}
			}
			\If{$status=EXECUTE \land hasLeftCriticalSection(aID())$}{
				\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\tcp*[r]{Explicit release}
				$status \gets NORMAL$\;
			}
		}
		
		\textbf{upon} $tryManeuver(turn)$ is invoked, do
		\Begin{				                              \lIf{$status \in \{NORMAL, GRANT\}$}{$tag \gets (clock(),aID(),turn)$}
			\uIf{$status \in \{NORMAL, TRYGET\}$}{
			    \textbf{let} $ts = clock()$\;
				$(status,AR,MR) \gets (TRYGET,(aID(), (ts,position(),velocity(),acceleration()),getMR(aID()))$\;
				\uIf{$(ts < MR[turn].tm + 2T_M \land MR[turn].MO)$}{
					$(\mathcal{M},\mathcal{D},\mathcal{R}, status) \gets (\bot,MR[turn].\mathcal{SM},MR[turn].\mathcal{SM}, GET)$\;
					\textbf{multicast} $\langle ts, GET, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
					$startTimer(T\_RETRY,2T_D)$\;
				}
				\lElse{$startTimer(T\_RETRY,T_A)$}
			}
			\lElseIf{$status=GRANT$}{$status \gets GRANTGET$}
		}
		\textbf{upon} timer $T\_RETRY$ expires
		\Begin{
			\If{$status=GET$}{
				$status \gets TRYGET$\;
				\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$\;
				$startTimer(T\_RETRY,2T_D)$\;
			}
			$tryManeuver(tag.turn)$\;
		}
		
		\textbf{upon} timer $T\_GRANT$ expires
		\Begin{
		    \textbf{let} $prevStatus = status$\;
			\If{$status \in \{GRANT, GRANTGET\} \land hasLeftCriticalSection(grantID)$}{$(status,grantID) \gets (NORMAL,\bot)$\; 
			    \lIf{$prevStatus = GRANTGET$}{
				    $tryManeuver()$}
		    }
			\lIf{$status \in \{GRANT, GRANTGET\}$}{$startTimer(T\_{GRANT},T_{Recover}$)}
			
		}
		
		\textbf{upon} message $m$ received at time $tr$
		\Begin{
			\If(\tcp*[f]{Message is timely}){$tr-m.t \leq T_D$}{
				\lIf{$m.type \in \{GRANT,DENY\} \land status=GET$}{
					$(\mathcal{M},\mathcal{R}) \gets (\mathcal{M} \cup \{m\},\mathcal{R} \setminus \{m.AR.aID\} )$
				}
				\uElseIf{$m.type=GET$}{
					\uIf{$noConflict(m.AR,m.AR.AS.ta + 2T_D + T_{MAN}) \land \newline (status\in\{NORMAL,TRYGET\} \lor (status=GET \land precedes(m.tag)) \lor \newline (status\in\{GRANT,GRANTGET\} \land grantID = m.AR.aID) )$}{
						\lIf{$status=NORMAL$}{$(status,grantID) \gets (GRANT,m.AR.aID)$}
						\ElseIf{$status \in \{GET,TRYGET\}$}{
							$stopTimer(T\_RETRY)$\;
							\lIf{$status=GET$}{\textbf{multicast} $\langle clock(), RELEASE, (AR, tag) \rangle$ \textbf{to} $\mathcal{D}$}
							$(status,grantID) \gets (GRANTGET,m.AR.aID)$\;
						}
						\textbf{send} $\langle tr, GRANT, \bot \rangle$ \textbf{to} $m.AR.aID$\;
						$startTimer(T\_GRANT, m.AR.AS.t + 2T_D + T_{MAN} - clock())$\; 
					}
					\lElse{\textbf{send} $\langle tr, DENY, \bot \rangle$ \textbf{to} $m.AR.aID$}
				}
				\ElseIf{$m.type=RELEASE \land status \in \{GRANT,GRANTGET\} \land grantID = m.AR.aID $}{
					$stopTimer(T\_GRANT)$\tcp*[r]{No need checking if an agent has left}
					$grantID \gets \bot$\;
					\lIf{$status=GRANT$}{$status \gets NORMAL$}
					\If{$status=GRANTGET$}{
						$status \gets TRYGET$\;
						$tryManeuver(tag.turn)$\;
					}
				}
			}
		}
		
	\end{footnotesize}
	\caption{The Manoeuvre Negotiation protocol}
	\label{alg:agent-events}
\end{algorithm}



==> include/backmatter/References.tex <==

\begin{thebibliography}{69}

\bibitem{Reference} Frisk, D. (2016) A Chalmers University of Technology Master's thesis template for \LaTeX . Unpublished.

\end{thebibliography}


==> include/frontmatter/Abstract.tex <==

An Informative Headline describing the Content of the Report\\
A Subtitle that can be Very Much Longer if Necessary\\
Emelie Ekenstedt\\
Department of Computer Science and Engineering\\
Chalmers University of Technology and University of Gothenburg\setlength{\parskip}{0.5cm}

\thispagestyle{plain}			% Supress header 
\setlength{\parskip}{0pt plus 1.0pt}
\section*{Abstract}

TBC

%The manoeuvre negotiation protocol is a protocol used by vehicles to negotiate their internal priority of getting access to the intersection.
%Used together with risk estimator...

% KEYWORDS (MAXIMUM 10 WORDS)
\vfill
Keywords: %Computer, science, computer science, engineering, project, thesis.

\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> include/frontmatter/Acknowledgements.tex <==

\thispagestyle{plain}			% Supress header
\section*{Acknowledgements}
Here, you can say thank you to your supervisor(s), company advisors and other people that supported you during your project.

\vspace{1.5cm}
\hfill
Emelie Ekenstedt, Gothenburg, June 2019

\newpage				% Create empty back of side
\thispagestyle{empty}
\mbox{}

==> include/frontmatter/Titlepage.tex <==

% COVER PAGE
\begin{titlepage}
\newgeometry{top=3cm, bottom=3cm,
			left=2.25 cm, right=2.25cm}	% Temporarily change margins		
			
% Cover page background 
\AddToShipoutPicture*{\backgroundpic{-4}{56.7}{figure/auxiliary/frontpage_gu_eng_vec_m2.pdf}}
\addtolength{\voffset}{2cm}

% Cover picture (replace with your own or delete)		
\begin{figure}[H]
\centering
\vspace{1cm}	% Adjust vertical spacing here
%\includegraphics[width=0.9\linewidth]{figure/somepicture}
\end{figure}

% Cover text
\mbox{}
\vfill
\renewcommand{\familydefault}{\sfdefault} \normalfont % Set cover page font
\textbf{{\Huge 	Membership-based Manoeuvre 	\\[0.2cm] 
			Negotiation in Autonomous and \\[0.2cm]
			Safety-critical Vehicular Systems}} 	\\[0.5cm]
%{\Large A Subtitle that can be Very Much Longer if Necessary}\\[0.5cm]
Master's thesis in Computer science and engineering \setlength{\parskip}{1cm}

{\Large Emelie Ekenstedt} \setlength{\parskip}{2.9cm}

Department of Computer Science and Engineering \\
\textsc{Chalmers University of Technology} \\
\textsc{University of Gothenburg} \\
Gothenburg, Sweden 2019

\renewcommand{\familydefault}{\rmdefault} \normalfont % Reset standard font
\end{titlepage}


% BACK OF COVER PAGE (BLANK PAGE)
\newpage
\restoregeometry
\thispagestyle{empty}
\mbox{}


% TITLE PAGE
\newpage
\thispagestyle{empty}
\begin{center}
	\textsc{\large Master's thesis 2019}\\[4cm]		% Report number is currently not in use
	\textbf{\Large An Informative Headline describing\\ the Content of the Report} \\[1cm]
	{\large A Subtitle that can be Very Much Longer if Necessary}\\[1cm]
	{\large Emelie Ekenstedt}
	
	\vfill	
	% Logotype on titlepage	
	\begin{figure}[H]
	\centering
	% Remove the following line to remove the titlepage logotype
	\includegraphics[width=0.25\pdfpagewidth]{figure/auxiliary/ChGULogoHog.pdf}
	\end{figure}	\vspace{5mm}	
	
	Department of Computer Science and Engineering\\
	%\emph{Division of Division name}\\
	%Name of research group (if applicable)\\
	\textsc{Chalmers University of Technology} \\
	\textsc{University of Gothenburg} \\
	Gothenburg, Sweden 2019 \\
\end{center}


% IMPRINT PAGE (BACK OF TITLE PAGE)
\newpage
\thispagestyle{plain}
\vspace*{4.5cm}
An Informative Headline describing the Content of the Report\\
A Subtitle that can be Very Much Longer if Necessary\\
Emelie Ekenstedt \setlength{\parskip}{1cm}

\copyright ~ Emelie Ekenstedt, 2019. \setlength{\parskip}{1cm}

Supervisor: Elad Schiller, Computer Science and Engineering\\
%Advisor: Name, Company or Institute (if applicable)\\
Examiner: Miquel Pericas, Computer Science and Engineering \setlength{\parskip}{1cm}

Master's Thesis 2019\\	% Report number currently not in use 
Department of Computer Science and Engineering\\
%Division of Division name\\
%Name of research group (if applicable)\\
Chalmers University of Technology and University of Gothenburg\\
SE-412 96 Gothenburg\\
Telephone +46 31 772 1000 \setlength{\parskip}{0.5cm}

\vfill
% Caption for cover page figure if used, possibly with reference to further information in the report
Cover: Description of the picture on the cover page (if applicable)


Typeset in \LaTeX \\
%Printed by [Name of printing company]\\
Gothenburg, Sweden 2019


